Scalar is Not Enough: Vectorization-based Unbiased Learning to Rank

Unbiased learning to rank (ULTR) aims to train an unbiased ranking model from biased user click logs. Most of the current ULTR methods are based on the examination hypothesis (EH), which assumes that the click probability can be factorized into two scalar functions, one related to ranking features and the other related to bias factors. Unfortunately, the interactions among features, bias factors and clicks are complicated in practice, and usually cannot be factorized in this independent way. Fitting click data with EH could lead to model misspecification and bring the approximation error. In this paper, we propose a vector-based EH and formulate the click probability as a dot product of two vector functions. This solution is complete due to its universality in fitting arbitrary click functions. Based on it, we propose a novel model named Vectorization to adaptively learn the relevance embeddings and sort documents by projecting embeddings onto a base vector. Extensive experiments show that our method significantly outperforms the state-of-the-art ULTR methods on complex real clicks as well as simple simulated clicks.

==> main_decouple.tex <==
\subsection{Decoupling}

\label{session_decoupling}

In this session, we will discuss two mechanisms to do soft decoupling under some conditions. Our basic idea is to control the capacity of the function $\predo{x}$, i.e., to make sure that the set of allowed parameters $\Theta^*$ defined in Assumption \ref{assumption_click_correct} is not too large, and then prove each function in this set achieve soft decoupling under some conditions. The proofs of the theorems in this section are provided in Appendix \sref{sec:proof}. From this point forward, we assume that all of the parameters $\theta$ take the value from $\Theta^*$, and omit $\theta$ of each estimation variable for ease of notation. 

\subsubsection{Lipschitz Decoupling}

\label{session_ld}

We start with defining the Lipschitz continuity for a function. Let $\norm{\cdot}$ be a norm on $\mathbb R^l$. In this work, we employ the Euclidean norm (L-2) when not mentioned otherwise: $\norm{\vx}=\norm[2]{\vx}=\sqrt{\sum_{i=1}^l x_i^2}$.

\begin{definition}[Lipschitz Continuity] A function $f(\vx): \sR^l\rightarrow \sR$ is $\alpha$-Lipschitz to the input $\vx$ if
$$
    |f(\vx')-f(\vx)|\leq \alpha \norm{\vx'-\vx},
$$
where $\alpha$ is referred to as the Lipschitz constant. 

\end{definition}

 Particularly, if an $\alpha-$Lipschitz function $f$ is differentiable, we have $\norm{\nabla_{\vx} f(\vx)} \leq \alpha$. We suppose $\realr{x},\realo{x},\predr{x}$ and $\predo{x}$ are all differentiable.


\begin{assumption}[True Observation Lipschitz]\label{assumption_real_propensity_smoothness} For each $p\in[n]$, the true observation $\realo{x}$ is $\alpha$-Lipschitz.
\end{assumption}

It assumes that there is an upper bound on the rate at which the true observation changes with the features. Similarly, we assume the observation estimation is also Lipschitz. We refer to this kind of observation model as \textbf{Lipschitz Observation Model} (LOM).


\begin{definition}[Lipschitz Observation Model] An observation model is $\beta-$Lipschitz observation model ($\beta$-LOM), if its estimation $\predo{x}$ is $\beta$-Lipschitz for all $p\in[n]$.

\end{definition}

We claim that soft decoupling can be achieved by selecting a lower $\beta$, as the following theorem.

\begin{theorem}[Lipschitz Decoupling] \label{theorem_smoothness_decoupling} For any two features $\vx_1$ and $\vx_2$, without loss of generality we suppose $\realr{x_1}\geq\realr{x_2}$. For a $\beta-$LOM, if the following condition is satisfied,
\begin{align*}
    \frac{\realr{x_1}}{\realr{x_2}}
    -1\geq
    \frac{\realo{x_1}}{\predeo{x_1}}
    \left\{\inf_{\gamma\in\Gamma} \int_{\gamma(\vx_1,\vx_2)}
        \frac
            {\beta\realo{x}+\alpha\predeo{x}}
            {o_p^2(\vx)}
        \norm{d\vx}
    \right\},    
\end{align*}

where $\Gamma(\vx_1,\vx_2)$ denotes the collection of all curves from point $\vx_1$ to point $\vx_2$. Then we have: $\preder{x_1}\geq\preder{x_2}$.

\end{theorem}

\begin{remark}

If the gap between $\realr{x_1}$ and $\realr{x_2}$ is large (i.e., $\frac{\realr{x_1}}{\realr{x_2}}$ is large) and $\alpha$ is small enough, there exists a $\beta$ such that the condition can be satisfied. Namely, when the true observation doesn't change too fast with the features, we can select a lower $\beta$ to achieve soft decoupling.
\end{remark}

At a high level, $\beta$-LOM controls the capacity of the function space $\Theta^*$ by restricting the Lipschitz constant $\beta$. While a low $\beta$ benefits the decoupling, it also suffers from the risk of underfitting. For example, if we adopt a $0-$LOM (known as Position-based Model) in the setting that the true observation has a large Lipschitz constant, we may not find a $\preder{x}$ and a $\predo{x}$ such that their product is equal to a given click rate $c_p(\vx)$. In other word, $\beta$ has a lower bound. This can be shown formally in the following theorem.

% From Theorem \ref{theorem_smoothness_decoupling}, one may conclude that forces an LOM model to have an extremely low Lipschitz constant (e.g., $\beta=0$) can get the best decoupling. However, it doesn't mean that $\beta$ can be as small as possible. When the real observation scores have a large Lipschitz constant, if we still force $\beta$ to small, we may not find $\preder{x}$ and $\predo{x}$ such that their product is equal to a given click rate $c_p(\vx)$. In other words, LOM with a low $\beta$ may be \textit{unsolvable} on a click dataset. This can be shown formally in the following theorem.

\begin{theorem}[Lower Bound of $\beta$] \label{theorem_LPM_solvability} Let $\vc(\vx)$ denote a vector containing click rates at each position:
$$
\vc({\vx})=\left(\realr{x}\realo[1]{\vx},\realr{x}\realo[2]{\vx},\dots,\realr{x}\realo[n]{\vx}\right)^\top.
$$
For any two different features $\vx_1$ and $\vx_2$, we have
$$
    \beta \geq \inf\limits_{t_1,t_2\geq1} 
    \frac
        {\norm[\infty]{
            t_1 \vc({\vx_1})-t_2 \vc({\vx_2})
        }}
        {\norm[2]{\vx_1-\vx_2}}.
$$
\end{theorem}

\begin{remark}
We consider a special situation where the true Observation is 0-Lipschitz ($\alpha=0$). In this case, we can find $t_1,t_2$ such that $t_1 \vc_{\vx_1}-t_2 \vc_{\vx_2}$ is a zero vector, and the lower bound of $\beta$ can be zero. When the true observation has a large Lipschitz number, $t_1 \vc_{\vx_1}-t_2 \vc_{\vx_2}$ can no longer be a zero vector and $\beta$ should be larger. It means the models should change quickly with the input feature to fit clicks.

\end{remark}

Theorem \ref{theorem_smoothness_decoupling} and Theorem \ref{theorem_LPM_solvability} give the upper bound and lower bound of $\beta$, respectively. In practice, we can tune the value of $\beta$ to achieve the best effect for soft decoupling. We refer to this method as \textbf{Lipschitz Decoupling}.

\subsubsection{Bernoulli Decoupling}


\label{session_bd}

Unfortunately, when $\alpha$ is large in a given dataset, it's difficult to select a proper $\beta$ such that the upper bound and the lower bound are satisfied at the same time. Under this circumstance, it may perform even worse than that without any debiasing operation (see \sref{sec_ex_diff_couple} for discussion). To address this problem, instead of making constraints on observation model's estimation, we explicitly add an additional sampling step for the generative process of $\rro$, as follows:
\begin{enumerate}
    \item Choose $\rro'\sim P(\cdot\mid\vrx,\rp;\theta_2)\in[0,1]$.
    \item Choose $\gamma\sim \text{Bernoulli}(1-t)$, where $0\leq t\leq 1$. Then $\rro = 1+(\rro'-1)\gamma$.
\end{enumerate}

% \begin{definition}[Bernoulli Observation Sampling] \label{def_bpm}
%     A $t-$Bernoulli Observation Sampling process ($t$-BPS, $0\leq t\leq 1$) generates $\rro$ in the following process:


% \end{definition}

That is to say, we randomly cancel the debiasing operation with a certain probability $t$ (i.e., force the observation model to predict $1$ as observation score and let the ranking model learn from clicks directly), to prevent it from getting worse when the true observation has a large Lipschitz constant. Now the sampling process of $\rro$ can be written as $\rro\sim P(\cdot\mid\vrx,\rp;\theta_2,t)$. Correspondingly, the estimation of observation model can be written as $\hat o_p(\vx; \theta_2,t)=\E(\rro\mid\vrx=\vx,\rp=p;\theta_2,t)$. Because all the previous assumptions don't limit the sampling process of $\rro$, the previous conclusions still hold in this new case. We define the observation model based on this new sampling process as $t$-\textbf{Bernoulli Observation Model} ($t$-BOM). 

% A $t$-BOM can be viewed as its intrinsic observation model whose output is powered by a Bernoulli random variable with parameter $1-t$. Particularly, a $0$-BOM is a normal observation model, and $1$-BOM is a observation model that will not debias click data. If the effects of relevance and observation are too coupled that debiasing will be counterproductive, we can increase $t$ to reduce the influence of the incorrect observation.
Next, we show how a BOM can achieve soft decoupling.

\begin{theorem}[Bernoulli Decoupling]\label{theorem_bernoulli_decoupling} For any two different features $\vx_1$ and $\vx_2$, without loss of generality we suppose $\realr{x_2}\geq\realr{x_1}$. For a $t-$BOM, if the following condition is satisfied,
$$
    t\geq % t<
    \frac{\realr{x_1}}{\realr{x_2}}  % x1/x2
    \left(
        1 + \frac
            {\alpha \norm{\vx_1-\vx_2}}
            {\sup\limits_{p} \realo{x_2}}
    \right),
$$
then we have: $\preder{x_2}\geq \preder{x_1}$.
\end{theorem}

\begin{remark}

If the true observation $\realo{x}$ is 0-Lipschitz (i.e., $\alpha=0$), there must exist a $t\leq1$ making the above error condition satisfied to achieve soft decoupling. For a larger Lipschitz number, we can increase the value of $t$ appropriately. 

\end{remark}

Similar to LOM, BOM is another method to control the capacity of $\Theta^*$, and it also suffers from the risk of underfitting. In order to make it fit the click rates, $t$ has an upper bound.

\begin{theorem}[Upper Bound of $t$] \label{theorem_bpm_solvability} For any feature $\vx$ and a $t-$BOM, we have
$$
    t\leq\frac{\inf\limits_{p} \realo[p]{x}}{\sup\limits_{p} \realo[p]{x}}.
$$
\end{theorem}
Theorem \ref{theorem_bernoulli_decoupling} and Theorem \ref{theorem_bpm_solvability} give the lower bound and the upper bound of $t$ respectively. Like LOM, we take $t$ as a tuning parameter in practice. We refer to this method as \textbf{Bernoulli Decoupling}.

% Besides, 

Finally, we propose our \textbf{$(\beta, t)$-Lipschitz and Bernoulli Decoupling} (LBD) model, which combines the $\beta$-LOM and $t$-BOM based on probabilistic ULTR framework. We treat LBD as our complete solution for individual-based ULTR.

